Single-participant structural connectivity matrices lead to greater accuracy in classification of participants than function in autism in MRI

In this work, we introduce a technique of deriving symmetric connectivity matrices from regional histograms of grey-matter volume estimated from T1-weighted MRIs. We then validated the technique by inputting the connectivity matrices into a convolutional neural network (CNN) to classify between participants with autism and age-, motion-, and intracranial-volume-matched controls from six different databases (29,288 total connectomes, mean age = 30.72, range 0.42-78.00, including 1555 subjects with autism). We compared this method to similar classifications of the same participants using fMRI connectivity matrices as well as univariate estimates of grey-matter volumes. We further applied graph-theoretical metrics on output class activation maps to identify areas of the matrices that the CNN preferentially used to make the classification, focusing particularly on hubs. Our results gave AUROCs of 0.7298 (69.71% accuracy) when classifying by only structural connectivity, 0.6964 (67.72% accuracy) when classifying by only functional connectivity, and 0.7037 (66.43% accuracy) when classifying by univariate grey matter volumes. Combining structural and functional connectivities gave an AUROC of 0.7354 (69.40% accuracy). Graph analysis of class activation maps revealed no distinguishable network patterns for functional inputs, but did reveal localized differences between groups in bilateral Heschl's gyrus and upper vermis for structural connectivity. This work provides a simple means of feature extraction for inputting large numbers of structural MRIs into machine learning models.

==> figures/age_collection_encoding.tex <==
\begin{figure}[t!]
\centering
\includegraphics[width=0.3\textwidth]{images/age_collection_encoding.png}
\caption{Sample array used to encode age and collection on the third layer of input. Every other line is the subject's age (scaled to be between 0 and 1) repeated, and every other line is a binary encoding of which collection the subject came from.}
\label{fig:age_collection_encoding}
\end{figure}

==> figures/asd_ensemble_model_projection.tex <==
\begin{figure}[t!]
\centering
\includegraphics[width=0.5\columnwidth]{images/ASD_Ensemble_Model_Projection.png}
\caption{Projection of the limit of the structure/function/age ensemble models, given data for ensembles of one to 300 models. Adding independent models \textit{ad infinitum} would result in a maximum predicted AUROC of 0.745.}
\label{fig:asd_ensemble_model_projection}
\end{figure}

==> figures/scatterplot_asd.tex <==
\begin{figure}[t!]
\centering
\includegraphics[width=0.5\textwidth]{images/scatterplot_asd.png}
\caption{Relative classification error in the structure/function/age ensemble model, plotted against age. Each point in the graph represents the averaged classification error of the datapoint across each model in which it was included in the test set. Thus, more controls are represented which were each used individually in fewer models, while the autism datasets are fewer but were generally used in more models. Thus represents that accuracy was generally higher in the developmental age groups, likely because more data was present for those groups.}
\label{fig:scatterplot_asd}
\end{figure}
